Kamino: Constraint-Aware Differentially Private Data Synthesis

Organizations are increasingly relying on data to support decisions. When data contains private and sensitive information, the data owner often desires to publish a synthetic database instance that is similarly useful as the true data, while ensuring the privacy of individual data records. Existing differentially private data synthesis methods aim to generate useful data based on applications, but they fail in keeping one of the most fundamental data properties of the structured data -- the underlying correlations and dependencies among tuples and attributes (i.e., the structure of the data). This structure is often expressed as integrity and schema constraints, or with a probabilistic generative process. As a result, the synthesized data is not useful for any downstream tasks that require this structure to be preserved. This work presents Kamino, a data synthesis system to ensure differential privacy and to preserve the structure and correlations present in the original dataset. Kamino takes as input of a database instance, along with its schema (including integrity constraints), and produces a synthetic database instance with differential privacy and structure preservation guarantees. We empirically show that while preserving the structure of the data, Kamino achieves comparable and even better usefulness in applications of training classification models and answering marginal queries than the state-of-the-art methods of differentially private data synthesis.

==> preprocess.tex <==
%!TEX root=./main.tex

\section{Constraint-Aware Pre-Processing}\label{sec:pre-processing}

Sections~\ref{sec:sequencing}-\ref{sec:sampling} present a general approach of our \system solution,
which relies on the computation model to learn the probability distributions.
In some cases, the computation model may not be able to learn accurately.
For example, when the true database instance have extremely large domain size, the discriminative models may not have sufficient support to learn the prediction.
Synthesizing data with large domain size is still an open problem, and existing solutions can only synthesize data with small domains. 

In this section, we present optimizations for extreme cases with respect to domain size:
1) a private filtering pre-processing when domain size is large;
and 2) a grouping technique when domain size is small.

\eat{
\subsubsection*{Pre-Processing for Large Domain Size}

To motivate the difficulty on synthesizing data with large domains, consider two attributes $zip$ and $state$ from the US tax dataset~\cite{DBLP:journals/pvldb/ChuIP13}.
The dataset has 30k rows, 10375 distinct zip codes, and 52 distinct states (and other jurisdictions).
Consider the FD $\phi_4$: $\forall t_i, t_j \in D$,
$\neg (t_i[zip]=t_j[zip] \land t_i[state] \neq t_j[state])$.
Given these information, the constraint-aware sequencing (Algorithm~\ref{alg:sequence}) will output a sequence starting with $zip$, and following $state$.
On average, each $zip$ appears in 3 rows, and it is likely some zips from the domain may not be sampled to train during the learning process
As a result, the discriminative model tends to randomly predicate $state$ values. 
However, in practice, $zip$ is not uniformly distributed.
For example, zip codes for metropolises are likely to be more frequent than ones for rural areas, for a given state.
In this case, to reduce the domain size for $zip$, we can keep the top-k most frequent zip codes per state, and categorize infrequent zip codes to one group.

\begin{algorithm}[h]
\caption{Constraint-aware frequent value filtering}\label{alg:freq}
\begin{algorithmic}[1]
\Require $D^*, \mathcal{D}$\Comment{True database instance, domain}
\Require $\phi, k, \beta$\Comment{Input FD, top-k frequent values, node fanout}
\Require $\epsilon_2$\Comment{DP budget}
\Procedure {Filtering}{$D^*, \mathcal{D}, \phi, k$}
\State $X, Y \gets$ lhs and rhs attribute of $\phi$
\State $\lambda \gets \frac{2\beta - 1}{\beta - 1} \times \frac{2}{\epsilon_2}$\label{alg:freq:pt_start}\Comment{Use $\frac{1}{2}\epsilon_2$ to decompose domains}
\State $\delta \gets \lambda \times \log{\beta}$\Comment{Decay factor~\cite{DBLP:conf/sigmod/ZhangXX16}}
\State Initialize a quadtree $\mathcal{T}$ with root node $v_1$
\State Set $v_1$'s 2D ranges as $\mathcal{D}[X]$ and $\mathcal{D}[Y]$
\State Mark $v_1$ unvisited
\While {there exists unvisited node $v$}
	\State Mark $v$ as visited
	\State $c(v) \gets$ counts of tuples falling within $c$'s domain
	\State $b(v) \gets c(v) - depth(v)\times \delta$
	\State $\hat{b}(v) \gets b(v) + Lap(\lambda)$
	\If {$\hat{b}(v) > 0$}
		\State Split $v$, add its unvisited children into $\mathcal{T}$
	\EndIf
\EndWhile\label{alg:freq:pt_end}
\State Initialize 2D array $C[|\mathcal{D}[X]|][|\mathcal{D}[Y]|] \gets \bf{0}$
\For{each leaf node $v\in \mathcal{T}$}
	\State $v$'s 2D ranges $Dom_X$ and $Dom_Y$
	\State $c\gets c(v) + Lap(\frac{2}{\epsilon_2})$\label{alg:freq:noisy-count}\Comment{Noisy counts with $\frac{1}{2}\epsilon_2$}
	\State $\hat{c} \gets \frac{\max(c, 0)}{|Dom_X|\times|Dom_Y|}$\Comment{Average counts}
	\State For each ($x,y$) in $v$'s range, increase $C[x][y]$ by $\hat{c}$
\EndFor
\State For each $x\in \mathcal{D}[X]$, return top-$k$ $ys$ from $C[x]$
\EndProcedure
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:freq} describes the process of finding top-k values from the second dimension $Y$ per each value in the first dimension $X$.
We adopt the PrivTree~\cite{DBLP:conf/sigmod/ZhangXX16} algorithm to partition the 2D space represented by a quad-tree~\cite{DBLP:books/daglib/0014978}, based on the lhs and rhs attributes of an FD (Line~\ref{alg:freq:pt_start}-\ref{alg:freq:pt_end}).
The idea is we partition the 2D space of domain into smaller partitions based on the density of tuples, whose data point falls into that region;
Within one partition, data points are assumed to be uniformly distributed, such that frequency of each points can be estimated.
For the given privacy budget $\epsilon_2$, we use half of it to create the private quad-tree (Line~\ref{alg:freq:pt_start}), and use the rest half to get noisy counts for each partition of the 2D domain range (Line~\ref{alg:freq:noisy-count}).
Algorithm~\ref{alg:freq} is $\epsilon_2$-DP, simply because of linear composition of two $\frac{1}{2}\epsilon_2$ algorithms.

This method can be further extended to include additional attributes. which are involved in DCs.
For example, consider we also have another FD
$\phi_5$: $\forall t_i, t_j \in D$,
$\neg (t_i[zip]=t_j[zip] \land t_i[city] \neq t_j[city])$,
which tells us $zip \rightarrow city$.
Algorithm~\ref{alg:freq} prunes out infrequent zips per state based on $\phi_4$,
and the corresponding cities can be pruned cascade, without incurring additional privacy loss.
}




